Towards End-to-End Acoustic Localization using Deep Learning: from Audio Signal to Source Position Coordinates

This paper presents a novel approach for indoor acoustic source localization using microphone arrays and based on a Convolutional Neural Network (CNN). The proposed solution is, to the best of our knowledge, the first published work in which the CNN is designed to directly estimate the three dimensional position of an acoustic source, using the raw audio signal as the input information avoiding the use of hand crafted audio features. Given the limited amount of available localization data, we propose in this paper a training strategy based on two steps. We first train our network using semi-synthetic data, generated from close talk speech recordings, and where we simulate the time delays and distortion suffered in the signal that propagates from the source to the array of microphones. We then fine tune this network using a small amount of real data. Our experimental results show that this strategy is able to produce networks that significantly improve existing localization methods based on \textit{SRP-PHAT} strategies. In addition, our experiments show that our CNN method exhibits better resistance against varying gender of the speaker and different window sizes compared with the other methods.

==> Definitions/journalnames.tex <==
\DeclareOption{acoustics}{	\gdef\@journal{acoustics}	\gdef\@journalshort{Acoustics}	\gdef\@journalfull{Acoustics}	\gdef\@doiabbr{acoustics}	\gdef\@ISSN{}	}
\DeclareOption{actuators}{	\gdef\@journal{actuators}	\gdef\@journalshort{Actuators}	\gdef\@journalfull{Actuators}	\gdef\@doiabbr{act}	\gdef\@ISSN{2076-0825}	}
\DeclareOption{addictions}{	\gdef\@journal{addictions}	\gdef\@journalshort{Addictions}	\gdef\@journalfull{Addictions}	\gdef\@doiabbr{}	\gdef\@ISSN{0006-0006}	}
\DeclareOption{admsci}{	\gdef\@journal{admsci}	\gdef\@journalshort{Adm. Sci.}	\gdef\@journalfull{Administrative Sciences}	\gdef\@doiabbr{admsci}	\gdef\@ISSN{2076-3387}	}
\DeclareOption{aerospace}{	\gdef\@journal{aerospace}	\gdef\@journalshort{Aerospace}	\gdef\@journalfull{Aerospace}	\gdef\@doiabbr{aerospace}	\gdef\@ISSN{2226-4310}	}
\DeclareOption{agriculture}{	\gdef\@journal{agriculture}	\gdef\@journalshort{Agriculture}	\gdef\@journalfull{Agriculture}	\gdef\@doiabbr{agriculture}	\gdef\@ISSN{2077-0472}	}
\DeclareOption{agronomy}{	\gdef\@journal{agronomy}	\gdef\@journalshort{Agronomy}	\gdef\@journalfull{Agronomy}	\gdef\@doiabbr{agronomy}	\gdef\@ISSN{2073-4395}	}
\DeclareOption{algorithms}{	\gdef\@journal{algorithms}	\gdef\@journalshort{Algorithms}	\gdef\@journalfull{Algorithms}	\gdef\@doiabbr{a}	\gdef\@ISSN{1999-4893}	}
\DeclareOption{animals}{	\gdef\@journal{animals}	\gdef\@journalshort{Animals}	\gdef\@journalfull{Animals}	\gdef\@doiabbr{ani}	\gdef\@ISSN{2076-2615}	}
\DeclareOption{antibiotics}{	\gdef\@journal{antibiotics}	\gdef\@journalshort{Antibiotics}	\gdef\@journalfull{Antibiotics}	\gdef\@doiabbr{antibiotics}	\gdef\@ISSN{2079-6382}	}
\DeclareOption{antibodies}{	\gdef\@journal{antibodies}	\gdef\@journalshort{Antibodies}	\gdef\@journalfull{Antibodies}	\gdef\@doiabbr{antib}	\gdef\@ISSN{2073-4468}	}
\DeclareOption{antioxidants}{	\gdef\@journal{antioxidants}	\gdef\@journalshort{Antioxidants}	\gdef\@journalfull{Antioxidants}	\gdef\@doiabbr{antiox}	\gdef\@ISSN{2076-3921}	}
\DeclareOption{applsci}{	\gdef\@journal{applsci}	\gdef\@journalshort{Appl. Sci.}	\gdef\@journalfull{Applied Sciences}	\gdef\@doiabbr{app}	\gdef\@ISSN{2076-3417}	}
\DeclareOption{arts}{	\gdef\@journal{arts}	\gdef\@journalshort{Arts}	\gdef\@journalfull{Arts}	\gdef\@doiabbr{arts}	\gdef\@ISSN{2076-0752}	}
\DeclareOption{asi}{	\gdef\@journal{asi}	\gdef\@journalshort{Appl. Syst. Innov.}	\gdef\@journalfull{Applied System Innovation}	\gdef\@doiabbr{asi}	\gdef\@ISSN{2571-5577}	}
\DeclareOption{atmosphere}{	\gdef\@journal{atmosphere}	\gdef\@journalshort{Atmosphere}	\gdef\@journalfull{Atmosphere}	\gdef\@doiabbr{atmos}	\gdef\@ISSN{2073-4433}	}
\DeclareOption{atoms}{	\gdef\@journal{atoms}	\gdef\@journalshort{Atoms}	\gdef\@journalfull{Atoms}	\gdef\@doiabbr{atoms}	\gdef\@ISSN{2218-2004}	}
\DeclareOption{axioms}{	\gdef\@journal{axioms}	\gdef\@journalshort{Axioms}	\gdef\@journalfull{Axioms}	\gdef\@doiabbr{axioms}	\gdef\@ISSN{2075-1680}	}
\DeclareOption{batteries}{	\gdef\@journal{batteries}	\gdef\@journalshort{Batteries}	\gdef\@journalfull{Batteries}	\gdef\@doiabbr{batteries}	\gdef\@ISSN{2313-0105}	}
\DeclareOption{bdcc}{	\gdef\@journal{bdcc}	\gdef\@journalshort{Big Data Cogn. Comput.}	\gdef\@journalfull{Big Data and Cognitive Computing}	\gdef\@doiabbr{bdcc}	\gdef\@ISSN{2504-2289}	}
\DeclareOption{behavsci}{ 	\gdef\@journal{behavsci} 	\gdef\@journalshort{Behav. Sci.}	\gdef\@journalfull{Behavioral Sciences}	\gdef\@doiabbr{bs}	\gdef\@ISSN{2076-328X}	}
\DeclareOption{beverages}{	\gdef\@journal{beverages}	\gdef\@journalshort{Beverages}	\gdef\@journalfull{Beverages}	\gdef\@doiabbr{beverages}	\gdef\@ISSN{2306-5710}	}
\DeclareOption{bioengineering}{	\gdef\@journal{bioengineering}	\gdef\@journalshort{Bioengineering}	\gdef\@journalfull{Bioengineering}	\gdef\@doiabbr{bioengineering}	\gdef\@ISSN{2306-5354}	}
\DeclareOption{biology}{	\gdef\@journal{biology}	\gdef\@journalshort{Biology}	\gdef\@journalfull{Biology}	\gdef\@doiabbr{biology}	\gdef\@ISSN{2079-7737}	}
\DeclareOption{biomedicines}{	\gdef\@journal{biomedicines}	\gdef\@journalshort{Biomedicines}	\gdef\@journalfull{Biomedicines}	\gdef\@doiabbr{biomedicines}	\gdef\@ISSN{2227-9059}	}
\DeclareOption{biomimetics}{	\gdef\@journal{biomimetics}	\gdef\@journalshort{Biomimetics}	\gdef\@journalfull{Biomimetics}	\gdef\@doiabbr{biomimetics}	\gdef\@ISSN{2313-7673}	}
\DeclareOption{biomolecules}{	\gdef\@journal{biomolecules}	\gdef\@journalshort{Biomolecules}	\gdef\@journalfull{Biomolecules}	\gdef\@doiabbr{biom}	\gdef\@ISSN{2218-273X}	}
\DeclareOption{biosensors}{	\gdef\@journal{biosensors}	\gdef\@journalshort{Biosensors}	\gdef\@journalfull{Biosensors}	\gdef\@doiabbr{bios}	\gdef\@ISSN{2079-6374}	}
\DeclareOption{brainsci}{ 	\gdef\@journal{brainsci} 	\gdef\@journalshort{Brain Sci.}	\gdef\@journalfull{Brain Sciences}	\gdef\@doiabbr{brainsci}	\gdef\@ISSN{2076-3425}	}
\DeclareOption{buildings}{	\gdef\@journal{buildings}	\gdef\@journalshort{Buildings}	\gdef\@journalfull{Buildings}	\gdef\@doiabbr{buildings}	\gdef\@ISSN{2075-5309}	}
\DeclareOption{cancers}{	\gdef\@journal{cancers}	\gdef\@journalshort{Cancers}	\gdef\@journalfull{Cancers}	\gdef\@doiabbr{cancers}	\gdef\@ISSN{2072-6694}	}
\DeclareOption{carbon}{ 	\gdef\@journal{carbon} 	\gdef\@journalshort{C}	\gdef\@journalfull{C}	\gdef\@doiabbr{c}	\gdef\@ISSN{2311-5629}	}
\DeclareOption{catalysts}{	\gdef\@journal{catalysts}	\gdef\@journalshort{Catalysts}	\gdef\@journalfull{Catalysts}	\gdef\@doiabbr{catal}	\gdef\@ISSN{2073-4344}	}
\DeclareOption{cells}{	\gdef\@journal{cells}	\gdef\@journalshort{Cells}	\gdef\@journalfull{Cells}	\gdef\@doiabbr{cells}	\gdef\@ISSN{2073-4409}	}
\DeclareOption{ceramics}{	\gdef\@journal{ceramics}	\gdef\@journalshort{Ceramics}	\gdef\@journalfull{Ceramics}	\gdef\@doiabbr{}	\gdef\@ISSN{2571-6131}	}
\DeclareOption{challenges}{	\gdef\@journal{challenges}	\gdef\@journalshort{Challenges}	\gdef\@journalfull{Challenges}	\gdef\@doiabbr{challe}	\gdef\@ISSN{2078-1547}	}
\DeclareOption{chemengineering}{	\gdef\@journal{chemengineering}	\gdef\@journalshort{ChemEngineering}	\gdef\@journalfull{ChemEngineering}	\gdef\@doiabbr{chemengineering}	\gdef\@ISSN{2305-7084}	}
\DeclareOption{chemosensors}{	\gdef\@journal{chemosensors}	\gdef\@journalshort{Chemosensors}	\gdef\@journalfull{Chemosensors}	\gdef\@doiabbr{chemosensors}	\gdef\@ISSN{2227-9040}	}
\DeclareOption{children}{	\gdef\@journal{children}	\gdef\@journalshort{Children}	\gdef\@journalfull{Children}	\gdef\@doiabbr{children}	\gdef\@ISSN{2227-9067}	}
\DeclareOption{cleantechnol}{	\gdef\@journal{cleantechnol}	\gdef\@journalshort{Clean Technol.}	\gdef\@journalfull{Clean Technologies}	\gdef\@doiabbr{cleantechnol}	\gdef\@ISSN{2571-8797}	}
\DeclareOption{climate}{	\gdef\@journal{climate}	\gdef\@journalshort{Climate}	\gdef\@journalfull{Climate}	\gdef\@doiabbr{cli}	\gdef\@ISSN{2225-1154}	}
\DeclareOption{clockssleep}{	\gdef\@journal{clockssleep}	\gdef\@journalshort{Clocks\&Sleep}	\gdef\@journalfull{Clocks \& Sleep}	\gdef\@doiabbr{clockssleep}	\gdef\@ISSN{2624-5175}	}
\DeclareOption{cmd}{	\gdef\@journal{cmd}	\gdef\@journalshort{Corros. Mater. Degrad.}	\gdef\@journalfull{Corrosion and Materials Degradation}	\gdef\@doiabbr{cmd}	\gdef\@ISSN{2000-4445}	}
\DeclareOption{coatings}{	\gdef\@journal{coatings}	\gdef\@journalshort{Coatings}	\gdef\@journalfull{Coatings}	\gdef\@doiabbr{coatings}	\gdef\@ISSN{2079-6412}	}
\DeclareOption{colloids}{	\gdef\@journal{colloids}	\gdef\@journalshort{Colloids Interfaces}	\gdef\@journalfull{Colloids Interfaces}	\gdef\@doiabbr{colloids}	\gdef\@ISSN{2504-5377}	}
\DeclareOption{computation}{	\gdef\@journal{computation}	\gdef\@journalshort{Computation}	\gdef\@journalfull{Computation}	\gdef\@doiabbr{computation}	\gdef\@ISSN{2079-3197}	}
\DeclareOption{computers}{	\gdef\@journal{computers}	\gdef\@journalshort{Computers}	\gdef\@journalfull{Computers}	\gdef\@doiabbr{computers}	\gdef\@ISSN{2073-431X}	}
\DeclareOption{condensedmatter}{	\gdef\@journal{condensedmatter}	\gdef\@journalshort{Condens. Matter}	\gdef\@journalfull{Condensed Matter}	\gdef\@doiabbr{condmat}	\gdef\@ISSN{2410-3896}	}
\DeclareOption{cosmetics}{	\gdef\@journal{cosmetics}	\gdef\@journalshort{Cosmetics}	\gdef\@journalfull{Cosmetics}	\gdef\@doiabbr{cosmetics}	\gdef\@ISSN{2079-9284}	}
\DeclareOption{cryptography}{	\gdef\@journal{cryptography}	\gdef\@journalshort{Cryptography}	\gdef\@journalfull{Cryptography}	\gdef\@doiabbr{cryptography}	\gdef\@ISSN{2410-387X}	}
\DeclareOption{crystals}{	\gdef\@journal{crystals}	\gdef\@journalshort{Crystals}	\gdef\@journalfull{Crystals}	\gdef\@doiabbr{cryst}	\gdef\@ISSN{2073-4352}	}
\DeclareOption{cybersecurity}{	\gdef\@journal{cybersecurity}	\gdef\@journalshort{Cybersecurity}	\gdef\@journalfull{Cybersecurity}	\gdef\@doiabbr{}	\gdef\@ISSN{0009-0009}	}
\DeclareOption{dairy}{	\gdef\@journal{dairy}	\gdef\@journalshort{Dairy}	\gdef\@journalfull{Dairy}	\gdef\@doiabbr{dairy}	\gdef\@ISSN{}	}
\DeclareOption{data}{	\gdef\@journal{data}	\gdef\@journalshort{Data}	\gdef\@journalfull{Data}	\gdef\@doiabbr{data}	\gdef\@ISSN{2306-5729}	}
\DeclareOption{dentistry}{	\gdef\@journal{dentistry}	\gdef\@journalshort{Dent. J.}	\gdef\@journalfull{Dentistry Journal}	\gdef\@doiabbr{dj}	\gdef\@ISSN{2304-6767}	}
\DeclareOption{designs}{ 	\gdef\@journal{designs} 	\gdef\@journalshort{Designs}	\gdef\@journalfull{Designs}	\gdef\@doiabbr{designs}	\gdef\@ISSN{2411-9660}	}
\DeclareOption{diagnostics}{	\gdef\@journal{diagnostics}	\gdef\@journalshort{Diagnostics}	\gdef\@journalfull{Diagnostics}	\gdef\@doiabbr{diagnostics}	\gdef\@ISSN{2075-4418}	}
\DeclareOption{diseases}{	\gdef\@journal{diseases}	\gdef\@journalshort{Diseases}	\gdef\@journalfull{Diseases}	\gdef\@doiabbr{diseases}	\gdef\@ISSN{2079-9721}	}
\DeclareOption{diversity}{	\gdef\@journal{diversity}	\gdef\@journalshort{Diversity}	\gdef\@journalfull{Diversity}	\gdef\@doiabbr{d}	\gdef\@ISSN{1424-2818}	}
\DeclareOption{drones}{	\gdef\@journal{drones}	\gdef\@journalshort{Drones}	\gdef\@journalfull{Drones}	\gdef\@doiabbr{drones}	\gdef\@ISSN{2504-446X}	}
\DeclareOption{econometrics}{	\gdef\@journal{econometrics}	\gdef\@journalshort{Econometrics}	\gdef\@journalfull{Econometrics}	\gdef\@doiabbr{econometrics}	\gdef\@ISSN{2225-1146}	}
\DeclareOption{economies}{	\gdef\@journal{economies}	\gdef\@journalshort{Economies}	\gdef\@journalfull{Economies}	\gdef\@doiabbr{economies}	\gdef\@ISSN{2227-7099}	}
\DeclareOption{education}{	\gdef\@journal{education}	\gdef\@journalshort{Educ. Sci.}	\gdef\@journalfull{Education Sciences}	\gdef\@doiabbr{educsci}	\gdef\@ISSN{2227-7102}	}
\DeclareOption{electrochem}{	\gdef\@journal{electrochem}	\gdef\@journalshort{Electrochem}	\gdef\@journalfull{Electrochem}	\gdef\@doiabbr{electrochem}	\gdef\@ISSN{}	}
\DeclareOption{electronics}{	\gdef\@journal{electronics}	\gdef\@journalshort{Electronics}	\gdef\@journalfull{Electronics}	\gdef\@doiabbr{electronics}	\gdef\@ISSN{2079-9292}	}
\DeclareOption{energies}{	\gdef\@journal{energies}	\gdef\@journalshort{Energies}	\gdef\@journalfull{Energies}	\gdef\@doiabbr{en}	\gdef\@ISSN{1996-1073}	}
\DeclareOption{entropy}{	\gdef\@journal{entropy}	\gdef\@journalshort{Entropy}	\gdef\@journalfull{Entropy}	\gdef\@doiabbr{e}	\gdef\@ISSN{1099-4300}	}
\DeclareOption{environments}{	\gdef\@journal{environments}	\gdef\@journalshort{Environments}	\gdef\@journalfull{Environments}	\gdef\@doiabbr{environments}	\gdef\@ISSN{2076-3298}	}
\DeclareOption{epigenomes}{	\gdef\@journal{epigenomes}	\gdef\@journalshort{Epigenomes}	\gdef\@journalfull{Epigenomes}	\gdef\@doiabbr{epigenomes}	\gdef\@ISSN{2075-4655}	}
\DeclareOption{est}{	\gdef\@journal{est}	\gdef\@journalshort{Electrochem. Sci. Technol.}	\gdef\@journalfull{Electrochemical Science and Technology}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{fermentation}{	\gdef\@journal{fermentation}	\gdef\@journalshort{Fermentation}	\gdef\@journalfull{Fermentation}	\gdef\@doiabbr{fermentation}	\gdef\@ISSN{2311-5637}	}
\DeclareOption{fibers}{	\gdef\@journal{fibers}	\gdef\@journalshort{Fibers}	\gdef\@journalfull{Fibers}	\gdef\@doiabbr{fib}	\gdef\@ISSN{2079-6439}	}
\DeclareOption{fire}{	\gdef\@journal{fire}	\gdef\@journalshort{Fire}	\gdef\@journalfull{Fire}	\gdef\@doiabbr{fire}	\gdef\@ISSN{2571-6255}	}
\DeclareOption{fishes}{	\gdef\@journal{fishes}	\gdef\@journalshort{Fishes}	\gdef\@journalfull{Fishes}	\gdef\@doiabbr{fishes}	\gdef\@ISSN{2410-3888}	}
\DeclareOption{fluids}{	\gdef\@journal{fluids}	\gdef\@journalshort{Fluids}	\gdef\@journalfull{Fluids}	\gdef\@doiabbr{fluids}	\gdef\@ISSN{2311-5521}	}
\DeclareOption{foods}{	\gdef\@journal{foods}	\gdef\@journalshort{Foods}	\gdef\@journalfull{Foods}	\gdef\@doiabbr{foods}	\gdef\@ISSN{2304-8158}	}
\DeclareOption{forecasting}{	\gdef\@journal{forecasting}	\gdef\@journalshort{Forecasting}	\gdef\@journalfull{Forecasting}	\gdef\@doiabbr{forecast}	\gdef\@ISSN{2571-9394}	}
\DeclareOption{forests}{	\gdef\@journal{forests}	\gdef\@journalshort{Forests}	\gdef\@journalfull{Forests}	\gdef\@doiabbr{f}	\gdef\@ISSN{1999-4907}	}
\DeclareOption{fractalfract}{	\gdef\@journal{fractalfract}	\gdef\@journalshort{Fractal Fract.}	\gdef\@journalfull{Fractal and Fractional}	\gdef\@doiabbr{fractalfract}	\gdef\@ISSN{2504-3110}	}
\DeclareOption{futureinternet}{	\gdef\@journal{futureinternet}	\gdef\@journalshort{Future Internet}	\gdef\@journalfull{Future Internet}	\gdef\@doiabbr{fi}	\gdef\@ISSN{1999-5903}	}
\DeclareOption{galaxies}{	\gdef\@journal{galaxies}	\gdef\@journalshort{Galaxies}	\gdef\@journalfull{Galaxies}	\gdef\@doiabbr{galaxies}	\gdef\@ISSN{2075-4434}	}
\DeclareOption{games}{	\gdef\@journal{games}	\gdef\@journalshort{Games}	\gdef\@journalfull{Games}	\gdef\@doiabbr{g}	\gdef\@ISSN{2073-4336}	}
\DeclareOption{gastrointestdisord}{	\gdef\@journal{gastrointestdisord}	\gdef\@journalshort{Gastrointest. Disord.}	\gdef\@journalfull{Gastrointestinal Disorders}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{gels}{	\gdef\@journal{gels}	\gdef\@journalshort{Gels}	\gdef\@journalfull{Gels}	\gdef\@doiabbr{gels}	\gdef\@ISSN{2310-2861}	}
\DeclareOption{genealogy}{	\gdef\@journal{genealogy}	\gdef\@journalshort{Genealogy}	\gdef\@journalfull{Genealogy}	\gdef\@doiabbr{genealogy}	\gdef\@ISSN{2313-5778}	}
\DeclareOption{genes}{	\gdef\@journal{genes}	\gdef\@journalshort{Genes}	\gdef\@journalfull{Genes}	\gdef\@doiabbr{genes}	\gdef\@ISSN{2073-4425}	}
\DeclareOption{geohazards}{	\gdef\@journal{geohazards}	\gdef\@journalshort{GeoHazards}	\gdef\@journalfull{GeoHazards}	\gdef\@doiabbr{geohazards}	\gdef\@ISSN{}	}
\DeclareOption{geosciences}{	\gdef\@journal{geosciences}	\gdef\@journalshort{Geosciences}	\gdef\@journalfull{Geosciences}	\gdef\@doiabbr{geosciences}	\gdef\@ISSN{2076-3263}	}
\DeclareOption{geriatrics}{	\gdef\@journal{geriatrics}	\gdef\@journalshort{Geriatrics}	\gdef\@journalfull{Geriatrics}	\gdef\@doiabbr{geriatrics}	\gdef\@ISSN{2308-3417}	}
\DeclareOption{hazardousmatters}{	\gdef\@journal{hazardousmatters}	\gdef\@journalshort{Hazard. Matters}	\gdef\@journalfull{Hazardous Matters}	\gdef\@doiabbr{}	\gdef\@ISSN{0014-0014}	}
\DeclareOption{healthcare}{	\gdef\@journal{healthcare}	\gdef\@journalshort{Healthcare}	\gdef\@journalfull{Healthcare}	\gdef\@doiabbr{healthcare}	\gdef\@ISSN{2227-9032}	}
\DeclareOption{heritage}{	\gdef\@journal{heritage}	\gdef\@journalshort{Heritage}	\gdef\@journalfull{Heritage}	\gdef\@doiabbr{heritage}	\gdef\@ISSN{2571-9408}	}
\DeclareOption{highthroughput}{	\gdef\@journal{highthroughput}	\gdef\@journalshort{High-Throughput}	\gdef\@journalfull{High-Throughput}	\gdef\@doiabbr{ht}	\gdef\@ISSN{2571-5135}	}
\DeclareOption{horticulturae}{	\gdef\@journal{horticulturae}	\gdef\@journalshort{Horticulturae}	\gdef\@journalfull{Horticulturae}	\gdef\@doiabbr{horticulturae}	\gdef\@ISSN{2311-7524}	}
\DeclareOption{humanities}{	\gdef\@journal{humanities}	\gdef\@journalshort{Humanities}	\gdef\@journalfull{Humanities}	\gdef\@doiabbr{h}	\gdef\@ISSN{2076-0787}	}
\DeclareOption{hydrology}{	\gdef\@journal{hydrology}	\gdef\@journalshort{Hydrology}	\gdef\@journalfull{Hydrology}	\gdef\@doiabbr{hydrology}	\gdef\@ISSN{2306-5338}	}
\DeclareOption{ijerph}{	\gdef\@journal{ijerph}	\gdef\@journalshort{Int. J. Environ. Res. Public Health}	\gdef\@journalfull{International Journal of Environmental Research and Public Health}	\gdef\@doiabbr{ijerph}	\gdef\@ISSN{1660-4601}	}
\DeclareOption{ijfs}{	\gdef\@journal{ijfs}	\gdef\@journalshort{Int. J. Financial Stud.}	\gdef\@journalfull{International Journal of Financial Studies}	\gdef\@doiabbr{ijfs}	\gdef\@ISSN{2227-7072}	}
\DeclareOption{ijgi}{	\gdef\@journal{ijgi}	\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}	\gdef\@journalfull{ISPRS International Journal of Geo-Information}	\gdef\@doiabbr{ijgi}	\gdef\@ISSN{2220-9964}	}
\DeclareOption{ijms}{	\gdef\@journal{ijms}	\gdef\@journalshort{Int. J. Mol. Sci.}	\gdef\@journalfull{International Journal of Molecular Sciences}	\gdef\@doiabbr{ijms}	\gdef\@ISSN{1422-0067}	}
\DeclareOption{ijtpp}{	\gdef\@journal{ijtpp}	\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}	\gdef\@journalfull{International Journal of Turbomachinery, Propulsion and Power}	\gdef\@doiabbr{ijtpp}	\gdef\@ISSN{2504-186X}	}
\DeclareOption{informatics}{	\gdef\@journal{informatics}	\gdef\@journalshort{Informatics}	\gdef\@journalfull{Informatics}	\gdef\@doiabbr{informatics}	\gdef\@ISSN{2227-9709}	}
\DeclareOption{information}{	\gdef\@journal{information}	\gdef\@journalshort{Information}	\gdef\@journalfull{Information}	\gdef\@doiabbr{info}	\gdef\@ISSN{2078-2489}	}
\DeclareOption{infrastructures}{	\gdef\@journal{infrastructures}	\gdef\@journalshort{Infrastructures}	\gdef\@journalfull{Infrastructures}	\gdef\@doiabbr{infrastructures}	\gdef\@ISSN{2412-3811}	}
\DeclareOption{inorganics}{	\gdef\@journal{inorganics}	\gdef\@journalshort{Inorganics}	\gdef\@journalfull{Inorganics}	\gdef\@doiabbr{inorganics}	\gdef\@ISSN{2304-6740}	}
\DeclareOption{insects}{	\gdef\@journal{insects}	\gdef\@journalshort{Insects}	\gdef\@journalfull{Insects}	\gdef\@doiabbr{insects}	\gdef\@ISSN{2075-4450}	}
\DeclareOption{instruments}{	\gdef\@journal{instruments}	\gdef\@journalshort{Instruments}	\gdef\@journalfull{Instruments}	\gdef\@doiabbr{instruments}	\gdef\@ISSN{2410-390X}	}
\DeclareOption{inventions}{	\gdef\@journal{inventions}	\gdef\@journalshort{Inventions}	\gdef\@journalfull{Inventions}	\gdef\@doiabbr{inventions}	\gdef\@ISSN{2411-5134}	}
\DeclareOption{j}{	\gdef\@journal{jjournal}	\gdef\@journalshort{J}	\gdef\@journalfull{J}	\gdef\@doiabbr{j}	\gdef\@ISSN{2571-8800}	}
\DeclareOption{jcdd}{	\gdef\@journal{jcdd}	\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}	\gdef\@journalfull{Journal of Cardiovascular Development and Disease}	\gdef\@doiabbr{jcdd}	\gdef\@ISSN{2308-3425}	}
\DeclareOption{jcm}{	\gdef\@journal{jcm}	\gdef\@journalshort{J. Clin. Med.}	\gdef\@journalfull{Journal of Clinical Medicine}	\gdef\@doiabbr{jcm}	\gdef\@ISSN{2077-0383}	}
\DeclareOption{jcs}{	\gdef\@journal{jcs}	\gdef\@journalshort{J. Compos. Sci.}	\gdef\@journalfull{Journal of Composites Science}	\gdef\@doiabbr{jcs}	\gdef\@ISSN{2504-477X}	}
\DeclareOption{jdb}{	\gdef\@journal{jdb}	\gdef\@journalshort{J. Dev. Biol.}	\gdef\@journalfull{Journal of Developmental Biology}	\gdef\@doiabbr{jdb}	\gdef\@ISSN{2221-3759}	}
\DeclareOption{jfb}{	\gdef\@journal{jfb}	\gdef\@journalshort{J. Funct. Biomater.}   	\gdef\@journalfull{Journal of Functional Biomaterials}   	\gdef\@doiabbr{jfb}	\gdef\@ISSN{2079-4983}	}
\DeclareOption{jfmk}{	\gdef\@journal{jfmk}	\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}   	\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}   	\gdef\@doiabbr{jfmk}	\gdef\@ISSN{2411-5142}	}
\DeclareOption{jimaging}{	\gdef\@journal{jimaging}	\gdef\@journalshort{J. Imaging}	\gdef\@journalfull{Journal of Imaging}	\gdef\@doiabbr{jimaging}	\gdef\@ISSN{2313-433X}	}
\DeclareOption{jintelligence}{	\gdef\@journal{jintelligence}	\gdef\@journalshort{J. Intell.}	\gdef\@journalfull{Journal of Intelligence}	\gdef\@doiabbr{jintelligence}	\gdef\@ISSN{2079-3200}	}
\DeclareOption{jlpea}{	\gdef\@journal{jlpea}	\gdef\@journalshort{J. Low Power Electron. Appl.}	\gdef\@journalfull{Journal of Low Power Electronics and Applications}	\gdef\@doiabbr{jlpea}	\gdef\@ISSN{2079-9268}	}
\DeclareOption{jmmp}{	\gdef\@journal{jmmp}	\gdef\@journalshort{J. Manuf. Mater. Process.}	\gdef\@journalfull{Journal of Manufacturing and Materials Processing}	\gdef\@doiabbr{jmmp}	\gdef\@ISSN{2504-4494}	}
\DeclareOption{jmse}{	\gdef\@journal{jmse}	\gdef\@journalshort{J. Mar. Sci. Eng.}	\gdef\@journalfull{Journal of Marine Science and Engineering}	\gdef\@doiabbr{jmse}	\gdef\@ISSN{2077-1312}	}
\DeclareOption{jof}{	\gdef\@journal{jof}	\gdef\@journalshort{J. Fungi}	\gdef\@journalfull{Journal of Fungi}	\gdef\@doiabbr{jof}	\gdef\@ISSN{2309-608X}	}
\DeclareOption{joitmc}{	\gdef\@journal{joitmc}	\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}	\gdef\@journalfull{Journal of Open Innovation: Technology, Market, and Complexity}	\gdef\@doiabbr{joitmc}	\gdef\@ISSN{2199-8531}	}
\DeclareOption{jpm}{	\gdef\@journal{jpm}	\gdef\@journalshort{J. Pers. Med.}	\gdef\@journalfull{Journal of Personalized Medicine}	\gdef\@doiabbr{jpm}	\gdef\@ISSN{2075-4426}	}
\DeclareOption{jrfm}{	\gdef\@journal{jrfm}	\gdef\@journalshort{J. Risk Financial Manag.}	\gdef\@journalfull{Journal of Risk and Financial Management}	\gdef\@doiabbr{jrfm}	\gdef\@ISSN{1911-8074}	}
\DeclareOption{jsan}{	\gdef\@journal{jsan}	\gdef\@journalshort{J. Sens. Actuator Netw.}	\gdef\@journalfull{Journal of Sensor and Actuator Networks}	\gdef\@doiabbr{jsan}	\gdef\@ISSN{2224-2708}	}
\DeclareOption{land}{	\gdef\@journal{land}	\gdef\@journalshort{Land}	\gdef\@journalfull{Land}	\gdef\@doiabbr{land}	\gdef\@ISSN{2073-445X}	}
\DeclareOption{languages}{	\gdef\@journal{languages}	\gdef\@journalshort{Languages}	\gdef\@journalfull{Languages}	\gdef\@doiabbr{languages}	\gdef\@ISSN{2226-471X}	}
\DeclareOption{laws}{	\gdef\@journal{laws}	\gdef\@journalshort{Laws}	\gdef\@journalfull{Laws}	\gdef\@doiabbr{laws}	\gdef\@ISSN{2075-471X}	}
\DeclareOption{life}{	\gdef\@journal{life}	\gdef\@journalshort{Life}	\gdef\@journalfull{Life}	\gdef\@doiabbr{life}	\gdef\@ISSN{2075-1729}	}
\DeclareOption{literature}{	\gdef\@journal{literature}	\gdef\@journalshort{Literature}	\gdef\@journalfull{Literature}	\gdef\@doiabbr{}	\gdef\@ISSN{2410-9789}	}
\DeclareOption{logistics}{	\gdef\@journal{logistics}	\gdef\@journalshort{Logistics}	\gdef\@journalfull{Logistics}	\gdef\@doiabbr{logistics}	\gdef\@ISSN{2305-6290}	}
\DeclareOption{lubricants}{	\gdef\@journal{lubricants}	\gdef\@journalshort{Lubricants}	\gdef\@journalfull{Lubricants}	\gdef\@doiabbr{lubricants}	\gdef\@ISSN{2075-4442}	}
\DeclareOption{machines}{	\gdef\@journal{machines}	\gdef\@journalshort{Machines}	\gdef\@journalfull{Machines}	\gdef\@doiabbr{machines}	\gdef\@ISSN{2075-1702}	}
\DeclareOption{magnetochemistry}{	\gdef\@journal{magnetochemistry}	\gdef\@journalshort{Magnetochemistry}	\gdef\@journalfull{Magnetochemistry}	\gdef\@doiabbr{magnetochemistry}	\gdef\@ISSN{2312-7481}	}
\DeclareOption{make}{	\gdef\@journal{make}	\gdef\@journalshort{Mach. Learn. Knowl. Extr.}	\gdef\@journalfull{Machine Learning and Knowledge Extraction}	\gdef\@doiabbr{make}	\gdef\@ISSN{2504-4990}	}
\DeclareOption{marinedrugs}{	\gdef\@journal{marinedrugs}	\gdef\@journalshort{Mar. Drugs}	\gdef\@journalfull{Marine Drugs}	\gdef\@doiabbr{md}	\gdef\@ISSN{1660-3397}	}
\DeclareOption{materials}{	\gdef\@journal{materials}	\gdef\@journalshort{Materials}	\gdef\@journalfull{Materials}	\gdef\@doiabbr{ma}	\gdef\@ISSN{1996-1944}	}
\DeclareOption{mathematics}{	\gdef\@journal{mathematics}	\gdef\@journalshort{Mathematics}	\gdef\@journalfull{Mathematics}	\gdef\@doiabbr{math}	\gdef\@ISSN{2227-7390}	}
\DeclareOption{mca}{	\gdef\@journal{mca}	\gdef\@journalshort{Math. Comput. Appl.}	\gdef\@journalfull{Mathematical and Computational Applications}	\gdef\@doiabbr{mca}	\gdef\@ISSN{2297-8747}	}
\DeclareOption{medicina}{	\gdef\@journal{medicina}	\gdef\@journalshort{Medicina}	\gdef\@journalfull{Medicina}	\gdef\@doiabbr{medicina}	\gdef\@ISSN{1010-660X}	}
\DeclareOption{medicines}{	\gdef\@journal{medicines}	\gdef\@journalshort{Medicines}	\gdef\@journalfull{Medicines}	\gdef\@doiabbr{medicines}	\gdef\@ISSN{2305-6320}	}
\DeclareOption{medsci}{	\gdef\@journal{medsci}	\gdef\@journalshort{Med. Sci.}	\gdef\@journalfull{Medical Sciences}	\gdef\@doiabbr{medsci}	\gdef\@ISSN{2076-3271}	}
\DeclareOption{membranes}{	\gdef\@journal{membranes}	\gdef\@journalshort{Membranes}	\gdef\@journalfull{Membranes}	\gdef\@doiabbr{membranes}	\gdef\@ISSN{2077-0375}	}
\DeclareOption{metabolites}{	\gdef\@journal{metabolites}	\gdef\@journalshort{Metabolites}	\gdef\@journalfull{Metabolites}	\gdef\@doiabbr{metabo}	\gdef\@ISSN{2218-1989}	}
\DeclareOption{metals}{	\gdef\@journal{metals}	\gdef\@journalshort{Metals}	\gdef\@journalfull{Metals}	\gdef\@doiabbr{met}	\gdef\@ISSN{2075-4701}	}
\DeclareOption{microarrays}{	\gdef\@journal{microarrays}	\gdef\@journalshort{Microarrays}	\gdef\@journalfull{Microarrays}	\gdef\@doiabbr{}	\gdef\@ISSN{2076-3905}	}
\DeclareOption{micromachines}{	\gdef\@journal{micromachines}	\gdef\@journalshort{Micromachines}	\gdef\@journalfull{Micromachines}	\gdef\@doiabbr{mi}	\gdef\@ISSN{2072-666X}	}
\DeclareOption{microorganisms}{	\gdef\@journal{microorganisms}	\gdef\@journalshort{Microorganisms}	\gdef\@journalfull{Microorganisms}	\gdef\@doiabbr{microorganisms}	\gdef\@ISSN{2076-2607}	}
\DeclareOption{minerals}{	\gdef\@journal{minerals}	\gdef\@journalshort{Minerals}	\gdef\@journalfull{Minerals}	\gdef\@doiabbr{min}	\gdef\@ISSN{2075-163X}	}
\DeclareOption{modelling}{	\gdef\@journal{modelling}	\gdef\@journalshort{Modelling}	\gdef\@journalfull{Modelling}	\gdef\@doiabbr{}	\gdef\@ISSN{0012-0012}	}
\DeclareOption{molbank}{	\gdef\@journal{molbank}	\gdef\@journalshort{Molbank}	\gdef\@journalfull{Molbank}	\gdef\@doiabbr{M}	\gdef\@ISSN{1422-8599}	}
\DeclareOption{molecules}{	\gdef\@journal{molecules}	\gdef\@journalshort{Molecules}	\gdef\@journalfull{Molecules}	\gdef\@doiabbr{molecules}	\gdef\@ISSN{1420-3049}	}
\DeclareOption{mps}{	\gdef\@journal{mps}	\gdef\@journalshort{Methods and Protoc.}	\gdef\@journalfull{Methods and Protocols}	\gdef\@doiabbr{mps}	\gdef\@ISSN{2409-9279}	}
\DeclareOption{mti}{	\gdef\@journal{mti}	\gdef\@journalshort{Multimodal Technologies and Interact.}	\gdef\@journalfull{Multimodal Technologies and Interaction}	\gdef\@doiabbr{mti}	\gdef\@ISSN{2414-4088}	}
\DeclareOption{nanomaterials}{	\gdef\@journal{nanomaterials}	\gdef\@journalshort{Nanomaterials}	\gdef\@journalfull{Nanomaterials}	\gdef\@doiabbr{nano}	\gdef\@ISSN{2079-4991}	}
\DeclareOption{ncrna}{	\gdef\@journal{ncrna}	\gdef\@journalshort{Non-coding RNA}	\gdef\@journalfull{Non-coding RNA}	\gdef\@doiabbr{ncrna}	\gdef\@ISSN{2311-553X}	}
\DeclareOption{neonatalscreening}{	\gdef\@journal{neonatalscreening}	\gdef\@journalshort{Int. J. Neonatal Screen.}	\gdef\@journalfull{International Journal of Neonatal Screening}	\gdef\@doiabbr{ijns}	\gdef\@ISSN{2409-515X}	}
\DeclareOption{neuroglia}{	\gdef\@journal{neuroglia}	\gdef\@journalshort{Neuroglia}	\gdef\@journalfull{Neuroglia}	\gdef\@doiabbr{neuroglia}	\gdef\@ISSN{2571-6980}	}
\DeclareOption{nitrogen}{	\gdef\@journal{nitrogen}	\gdef\@journalshort{Nitrogen}	\gdef\@journalfull{Nitrogen}	\gdef\@doiabbr{nitrogen}	\gdef\@ISSN{2504-3129}	}
\DeclareOption{notspecified}{	\gdef\@journal{notspecified}	\gdef\@journalshort{Journal Not Specified}	\gdef\@journalfull{Journal Not Specified}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{nutrients}{	\gdef\@journal{nutrients}	\gdef\@journalshort{Nutrients}	\gdef\@journalfull{Nutrients}	\gdef\@doiabbr{nu}	\gdef\@ISSN{2072-6643}	}
\DeclareOption{ohbm}{	\gdef\@journal{ohbm}	\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}	\gdef\@journalfull{Journal of Otorhinolaryngology, Hearing and Balance Medicine}	\gdef\@doiabbr{ohbm}	\gdef\@ISSN{2504-463X}	}
\DeclareOption{particles}{	\gdef\@journal{particles}	\gdef\@journalshort{Particles}	\gdef\@journalfull{Particles}	\gdef\@doiabbr{particles}	\gdef\@ISSN{2571-712X}	}
\DeclareOption{pathogens}{	\gdef\@journal{pathogens}	\gdef\@journalshort{Pathogens}	\gdef\@journalfull{Pathogens}	\gdef\@doiabbr{pathogens}	\gdef\@ISSN{2076-0817}	}
\DeclareOption{pharmaceuticals}{	\gdef\@journal{pharmaceuticals}	\gdef\@journalshort{Pharmaceuticals}	\gdef\@journalfull{Pharmaceuticals}	\gdef\@doiabbr{ph}	\gdef\@ISSN{1424-8247}	}
\DeclareOption{pharmaceutics}{	\gdef\@journal{pharmaceutics}	\gdef\@journalshort{Pharmaceutics}	\gdef\@journalfull{Pharmaceutics}	\gdef\@doiabbr{pharmaceutics}	\gdef\@ISSN{1999-4923}	}
\DeclareOption{pharmacy}{	\gdef\@journal{pharmacy}	\gdef\@journalshort{Pharmacy}	\gdef\@journalfull{Pharmacy}	\gdef\@doiabbr{pharmacy}	\gdef\@ISSN{2226-4787}	}
\DeclareOption{philosophies}{	\gdef\@journal{philosophies}	\gdef\@journalshort{Philosophies}	\gdef\@journalfull{Philosophies}	\gdef\@doiabbr{philosophies}	\gdef\@ISSN{2409-9287}	}
\DeclareOption{photonics}{	\gdef\@journal{photonics}	\gdef\@journalshort{Photonics}	\gdef\@journalfull{Photonics}	\gdef\@doiabbr{photonics}	\gdef\@ISSN{2304-6732}	}
\DeclareOption{plants}{	\gdef\@journal{plants}	\gdef\@journalshort{Plants}	\gdef\@journalfull{Plants}	\gdef\@doiabbr{plants}	\gdef\@ISSN{2223-7747}	}
\DeclareOption{plasma}{	\gdef\@journal{plasma}	\gdef\@journalshort{Plasma}	\gdef\@journalfull{Plasma}	\gdef\@doiabbr{plasma}	\gdef\@ISSN{2571-6182}	}
\DeclareOption{polymers}{	\gdef\@journal{polymers}	\gdef\@journalshort{Polymers}	\gdef\@journalfull{Polymers}	\gdef\@doiabbr{polym}	\gdef\@ISSN{2073-4360}	}
\DeclareOption{polysaccharides}{	\gdef\@journal{polysaccharides}	\gdef\@journalshort{Polysaccharides}	\gdef\@journalfull{Polysaccharides}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{preprints}{ 	\gdef\@journal{preprints} 	\gdef\@journalshort{Preprints}	\gdef\@journalfull{Preprints}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{proceedings}{	\gdef\@journal{proceedings}	\gdef\@journalshort{Proceedings}	\gdef\@journalfull{Proceedings}	\gdef\@doiabbr{proceedings}	\gdef\@ISSN{2504-3900}	}
\DeclareOption{processes}{	\gdef\@journal{processes}	\gdef\@journalshort{Processes}	\gdef\@journalfull{Processes}	\gdef\@doiabbr{pr}	\gdef\@ISSN{2227-9717}	}
\DeclareOption{proteomes}{	\gdef\@journal{proteomes}	\gdef\@journalshort{Proteomes}	\gdef\@journalfull{Proteomes}	\gdef\@doiabbr{proteomes}	\gdef\@ISSN{2227-7382}	}
\DeclareOption{publications}{	\gdef\@journal{publications}	\gdef\@journalshort{Publications}	\gdef\@journalfull{Publications}	\gdef\@doiabbr{publications}	\gdef\@ISSN{2304-6775}	}
\DeclareOption{quaternary}{	\gdef\@journal{quaternary}	\gdef\@journalshort{Quaternary}	\gdef\@journalfull{Quaternary}	\gdef\@doiabbr{quat}	\gdef\@ISSN{2571-550X}	}
\DeclareOption{qubs}{	\gdef\@journal{qubs}	\gdef\@journalshort{Quantum Beam Sci.}	\gdef\@journalfull{Quantum Beam Science}	\gdef\@doiabbr{qubs}	\gdef\@ISSN{2412-382X}	}
\DeclareOption{reactions}{	\gdef\@journal{reactions}	\gdef\@journalshort{Reactions}	\gdef\@journalfull{Reactions}	\gdef\@doiabbr{reactions}	\gdef\@ISSN{}	}
\DeclareOption{recycling}{	\gdef\@journal{recycling}	\gdef\@journalshort{Recycling}	\gdef\@journalfull{Recycling}	\gdef\@doiabbr{recycling}	\gdef\@ISSN{2313-4321}	}
\DeclareOption{religions}{	\gdef\@journal{religions}	\gdef\@journalshort{Religions}	\gdef\@journalfull{Religions}	\gdef\@doiabbr{rel}	\gdef\@ISSN{2077-1444}	}
\DeclareOption{remotesensing}{	\gdef\@journal{remotesensing}	\gdef\@journalshort{Remote Sens.}	\gdef\@journalfull{Remote Sensing}	\gdef\@doiabbr{rs}	\gdef\@ISSN{2072-4292}	}
\DeclareOption{reports}{	\gdef\@journal{reports}	\gdef\@journalshort{Reports}	\gdef\@journalfull{Reports}	\gdef\@doiabbr{reports}	\gdef\@ISSN{2571-841X}	}
\DeclareOption{resources}{	\gdef\@journal{resources}	\gdef\@journalshort{Resources}	\gdef\@journalfull{Resources}	\gdef\@doiabbr{resources}	\gdef\@ISSN{2079-9276}	}
\DeclareOption{risks}{	\gdef\@journal{risks}	\gdef\@journalshort{Risks}	\gdef\@journalfull{Risks}	\gdef\@doiabbr{risks}	\gdef\@ISSN{2227-9091}	}
\DeclareOption{robotics}{	\gdef\@journal{robotics}	\gdef\@journalshort{Robotics}	\gdef\@journalfull{Robotics}	\gdef\@doiabbr{robotics}	\gdef\@ISSN{2218-6581}	}
\DeclareOption{safety}{	\gdef\@journal{safety}	\gdef\@journalshort{Safety}	\gdef\@journalfull{Safety}	\gdef\@doiabbr{safety}	\gdef\@ISSN{2313-576X}	}
\DeclareOption{sci}{	\gdef\@journal{sci}	\gdef\@journalshort{Sci}	\gdef\@journalfull{Sci}	\gdef\@doiabbr{}	\gdef\@ISSN{2413-4155}	}
\DeclareOption{scipharm}{	\gdef\@journal{scipharm}	\gdef\@journalshort{Sci. Pharm.}	\gdef\@journalfull{Scientia Pharmaceutica}	\gdef\@doiabbr{scipharm}	\gdef\@ISSN{2218-0532}	}
\DeclareOption{sensors}{	\gdef\@journal{sensors}	\gdef\@journalshort{Sensors}	\gdef\@journalfull{Sensors}	\gdef\@doiabbr{s}	\gdef\@ISSN{1424-8220}	}
\DeclareOption{separations}{	\gdef\@journal{separations}	\gdef\@journalshort{Separations}	\gdef\@journalfull{Separations}	\gdef\@doiabbr{separations}	\gdef\@ISSN{2297-8739}	}
\DeclareOption{sexes}{	\gdef\@journal{sexes}	\gdef\@journalshort{Sexes}	\gdef\@journalfull{Sexes}	\gdef\@doiabbr{}	\gdef\@ISSN{2411-5118}	}
\DeclareOption{sinusitis}{	\gdef\@journal{sinusitis}	\gdef\@journalshort{Sinusitis}	\gdef\@journalfull{Sinusitis}	\gdef\@doiabbr{sinusitis}	\gdef\@ISSN{2309-107X}	}
\DeclareOption{smartcities}{	\gdef\@journal{smartcities}	\gdef\@journalshort{Smart Cities}	\gdef\@journalfull{Smart Cities}	\gdef\@doiabbr{smartcities}	\gdef\@ISSN{}	}
\DeclareOption{societies}{	\gdef\@journal{societies}	\gdef\@journalshort{Societies}	\gdef\@journalfull{Societies}	\gdef\@doiabbr{soc}	\gdef\@ISSN{2075-4698}	}
\DeclareOption{socsci}{	\gdef\@journal{socsci}	\gdef\@journalshort{Soc. Sci.}	\gdef\@journalfull{Social Sciences}	\gdef\@doiabbr{socsci}	\gdef\@ISSN{2076-0760}	}
\DeclareOption{soilsystems}{	\gdef\@journal{soilsystems}	\gdef\@journalshort{Soil Syst.}	\gdef\@journalfull{Soil Systems}	\gdef\@doiabbr{soilsystems}	\gdef\@ISSN{2571-8789}	}
\DeclareOption{sports}{	\gdef\@journal{sports}	\gdef\@journalshort{Sports}	\gdef\@journalfull{Sports}	\gdef\@doiabbr{sports}	\gdef\@ISSN{2075-4663}	}
\DeclareOption{standards}{	\gdef\@journal{standards}	\gdef\@journalshort{Standards}	\gdef\@journalfull{Standards}	\gdef\@doiabbr{}	\gdef\@ISSN{2305-6703}	}
\DeclareOption{stats}{	\gdef\@journal{stats}	\gdef\@journalshort{Stats}	\gdef\@journalfull{Stats}	\gdef\@doiabbr{stats}	\gdef\@ISSN{2571-905X}	}
\DeclareOption{surfaces}{	\gdef\@journal{surfaces}	\gdef\@journalshort{Surfaces}	\gdef\@journalfull{Surfaces}	\gdef\@doiabbr{surfaces}	\gdef\@ISSN{2571-9637}	}
\DeclareOption{surgeries}{	\gdef\@journal{surgeries}	\gdef\@journalshort{Surgeries}	\gdef\@journalfull{Surgeries}	\gdef\@doiabbr{}	\gdef\@ISSN{2017-2017}	}
\DeclareOption{sustainability}{	\gdef\@journal{sustainability}	\gdef\@journalshort{Sustainability}	\gdef\@journalfull{Sustainability}	\gdef\@doiabbr{su}	\gdef\@ISSN{2071-1050}	}
\DeclareOption{symmetry}{	\gdef\@journal{symmetry}	\gdef\@journalshort{Symmetry}	\gdef\@journalfull{Symmetry}	\gdef\@doiabbr{sym}	\gdef\@ISSN{2073-8994}	}
\DeclareOption{systems}{	\gdef\@journal{systems}	\gdef\@journalshort{Systems}	\gdef\@journalfull{Systems}	\gdef\@doiabbr{systems}	\gdef\@ISSN{2079-8954}	}
\DeclareOption{technologies}{	\gdef\@journal{technologies}	\gdef\@journalshort{Technologies}	\gdef\@journalfull{Technologies}	\gdef\@doiabbr{technologies}	\gdef\@ISSN{2227-7080}	}
\DeclareOption{test}{	\gdef\@journal{test}	\gdef\@journalshort{Test}	\gdef\@journalfull{Test}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{toxics}{	\gdef\@journal{toxics}	\gdef\@journalshort{Toxics}	\gdef\@journalfull{Toxics}	\gdef\@doiabbr{toxics}	\gdef\@ISSN{2305-6304}	}
\DeclareOption{toxins}{	\gdef\@journal{toxins}	\gdef\@journalshort{Toxins}	\gdef\@journalfull{Toxins}	\gdef\@doiabbr{toxins}	\gdef\@ISSN{2072-6651}	}
\DeclareOption{tropicalmed}{	\gdef\@journal{tropicalmed}	\gdef\@journalshort{Trop. Med. Infect. Dis.}	\gdef\@journalfull{Tropical Medicine and Infectious Disease}	\gdef\@doiabbr{tropicalmed}	\gdef\@ISSN{2414-6366}	}
\DeclareOption{universe}{	\gdef\@journal{universe}	\gdef\@journalshort{Universe}	\gdef\@journalfull{Universe}	\gdef\@doiabbr{universe}	\gdef\@ISSN{2218-1997}	}
\DeclareOption{urbansci}{	\gdef\@journal{urbansci}	\gdef\@journalshort{Urban Sci.}	\gdef\@journalfull{Urban Science}	\gdef\@doiabbr{urbansci}	\gdef\@ISSN{2413-8851}	}
\DeclareOption{vaccines}{	\gdef\@journal{vaccines}	\gdef\@journalshort{Vaccines}	\gdef\@journalfull{Vaccines}	\gdef\@doiabbr{vaccines}	\gdef\@ISSN{2076-393X}	}
\DeclareOption{vehicles}{	\gdef\@journal{vehicles}	\gdef\@journalshort{Vehicles}	\gdef\@journalfull{Vehicles}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{vetsci}{	\gdef\@journal{vetsci}	\gdef\@journalshort{Vet. Sci.}	\gdef\@journalfull{Veterinary Sciences}	\gdef\@doiabbr{vetsci}	\gdef\@ISSN{2306-7381}	}
\DeclareOption{vibration}{	\gdef\@journal{vibration}	\gdef\@journalshort{Vibration}	\gdef\@journalfull{Vibration}	\gdef\@doiabbr{vibration}	\gdef\@ISSN{2571-631X}	}
\DeclareOption{viruses}{	\gdef\@journal{viruses}	\gdef\@journalshort{Viruses}	\gdef\@journalfull{Viruses}	\gdef\@doiabbr{v}	\gdef\@ISSN{1999-4915}	}
\DeclareOption{vision}{	\gdef\@journal{vision}	\gdef\@journalshort{Vision}	\gdef\@journalfull{Vision}	\gdef\@doiabbr{vision}	\gdef\@ISSN{2411-5150}	}
\DeclareOption{water}{	\gdef\@journal{water}	\gdef\@journalshort{Water}	\gdef\@journalfull{Water}	\gdef\@doiabbr{w}	\gdef\@ISSN{2073-4441}	}
\DeclareOption{wem}{	\gdef\@journal{wem}	\gdef\@journalshort{Wildl. Ecol. Manag.}	\gdef\@journalfull{Wildlife Ecology and Management}	\gdef\@doiabbr{}	\gdef\@ISSN{1234-4321}	}
\DeclareOption{wevj}{	\gdef\@journal{wevj}	\gdef\@journalshort{World Electric Vehicle Journal}	\gdef\@journalfull{World Electric Vehicle Journal}	\gdef\@doiabbr{wevj}	\gdef\@ISSN{}	}

==> system-description-old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{System description}

% In this section, we introduce our convolutional neural network proposal for estimating the position of an acoustic source from the given raw audio signals recorded by microphone arrays located inside a room. The network topology implements an end-to-end system if the form
% %The main objective of this paper is to obtain a spatial position vector of a speaker from the raw audio input signals recorded by some known located microphones inside a room. Equation \ref{eq:eqsystem} summarize the function to be accomplished by the system, where $s_{mic_{i}}[n]$ denotes the raw audio signal captured by each microphone and the vector $(x, y, z)$ the spatial coordinates of the estimated speaker's position.

% \begin{equation} \label{eq:eqsystem}
% (x, y, z) = f(s_{mic_{1}}[n], s_{mic_{2}}[n], \dots , s_{mic_{N}}[n])  
% \end{equation}

% %The \textit{IDIAP} research institute \textit{Smart Meeting Room} \cite{lathoud2005av16} layout have been used as our testing room, which is a $3.6m \times 8.2m \times 2.4m$ rectangular room with a rectangular table centrally located $4.8m \times 1.2m$ size. On the table's surface there are two circular microphone arrays of $0.1m$ radius, each composed by 8 equidistant microphones as shown in figure \ref{fig:IdiapSettings}. The centers of both arrays are separated by $0.8m$, where the middle point between them is considered as the origin of coordinates. In this proposal, only the microphones 1, 5, 11 and 15 are enabled and the used set up for them is shown in figure \ref{fig:IdiapSettings} c.

% \begin{figure}[H]
% 	\begin{tabular}{ccc}

% 		\includegraphics[width=0.32\textwidth]{figures/RoomSet-Up.png}
% 		& \includegraphics[width=0.32\textwidth]{figures/RoomExample.png}
% 		& \includegraphics[width=0.15\textwidth]{figures/MicSetUp.png}\\
% 		\textbf{(a)} & \textbf{(b)} & \textbf{(c)}

% 	\end{tabular}
% 	\caption{ \textit{IDIAP Smart Meeting Room} layout (a), a real example of the room extracted from a video frame (b) and the set up used in this proposal}
% 	\label{fig:IdiapSettings}
% \end{figure}

% In order to achieve the proposed goal, we have implemented a simple convolutional neural network which, from the four used microphones raw audio signals, will be able to approach the system function obtaining the best performance on giving the estimated spatial position vector.

% \subsection{Network Topology}
% The neural network topology we propose is shown in figure \ref{fig:NetScheme} which is composed by five convolutional blocks of one dimension and a fully connected block. The input of the system are the four time windowed signals of each used microphones and its output is the estimated $(x, y, z)$ position vector of the acoustic source.

% \begin{figure}[H]
% 	\centering
% 	\includegraphics[width=0.8\textwidth]{figures/NetScheme1D.png}
% 	\caption{Used network topology}
% 	\label{fig:NetScheme}
% \end{figure}

% The first convolutional block has 96 filters with 7 coefficients each followed by a \textit{MaxPooling} layers with a 7 pool size. The second convolutional block is composed by 96 filters with 7 coefficients as well. The third and the fourth convolutional blocks have 128 filters with 7 coefficients where the first of them is followed by a \textit{MaxPooling} layer of 5 pool size while the second is followed by a 3 pool size \textit{MaxPooling} layer and he fifth convolutional block only has 128 filters with 3 coefficients each. The last layer is a 500 nodes fully connected layer with a dropout of $0.5$. 

% \begin{table}[H]
% 	\centering
% 	\begin{tabular}{c|c|c}
%     	\textbf{Block} & \textbf{Filters} & \textbf{Kernel}\\
%         \midrule
%         Convolutional block 1 & 96 & 7 \\
%         \midrule
%         Convolutional block 2 & 96 & 7 \\
%         \midrule
%         Convolutional block 3 & 128 & 5 \\
%         \midrule
%         Convolutional block 4 & 128 & 5 \\
%         \midrule
%         Convolutional block 5 & 128 & 3 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Network convolutional layers summary}
%     \label{tab:NetworkLayers}
% \end{table}


==> table-SRPresults.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c|c|c|c}
		\toprule
		& \textbf{80$ms$}	& \textbf{160$ms$} & \textbf{320$ms$}\\
		\midrule
		seq01 & $MOTP$ = 1.02m & $MOTP$ = 0.91m & $MOTP$ = 0.83m\\
		\midrule
		seq02 & $MOTP$ = 0.96m & $MOTP$ = 0.84m & $MOTP$ = 0.77m\\
		\midrule
		seq03 & $MOTP$ = 0.90m & $MOTP$ = 0.77m & $MOTP$ = 0.69m\\
	\end{tabular}
	\caption{Baseline $MOTP(m)$ results for sequences \texttt{seq1},
    \texttt{seq2} and \texttt{seq3}, for different window sizes.} 
	\label{tab:SRPResults}
\end{table}


==> table-baseline+ft15+1+2+3-withsrp.tex <==
\begin{table}[H]
\footnotesize
	\centering
	\begin{tabular}{c|ccc|ccc|ccc}
%		\hline
    &   \multicolumn{3}{c|}{\textbf{80$ms$}}	& \multicolumn{3}{c|}{\textbf{160$ms$}} & \multicolumn{3}{c}{\textbf{320$ms$}}\\
    &   SRP & GMBF & CNNf15+static & SRP & GMBF & CNNf15+static & SRP & GMBF & CNNf15+static \\\hline\hline
\multirow{2}{*}{\seq01 \legendMOTPDelta} & $1.020$ & $0.795$ & $\mbf{0.619}$ & $0.910$ & $0.686$ & $\mbf{0.570}$ & $0.830$ & $0.588$ & $\mbf{0.493}$\\
 &  & $22.1\%$ & $\mbf{39.3\%}$ &  & $24.6\%$ & $\mbf{37.4\%}$ &  & $29.1\%$ & $\mbf{40.6\%}$ \\\hline
\multirow{2}{*}{\seq02 \legendMOTPDelta} & $0.960$ & $0.864$ & $\mbf{0.685}$ & $0.840$ & $0.759$ & $\mbf{0.603}$ & $0.770$ & $0.694$ & $\mbf{0.554}$ \\
 &  & $10.0\%$ & $\mbf{28.6\%}$ &  & $9.6\%$ & $\mbf{28.2\%}$ &  & $9.9\%$ & $\mbf{28.1\%}$ \\\hline
\multirow{2}{*}{\seq03 \legendMOTPDelta} & $0.900$ & $\mbf{0.686}$ & $0.694$ & $0.770$ & $\mbf{0.563}$ & $0.638$ & $0.690$ & $\mbf{0.484}$ & $0.540$ \\
 &  & $\mbf{23.8\%}$ & $22.9\%$ &  & $\mbf{26.9\%}$ & $17.1\%$ &  & $\mbf{29.9\%}$ & $21.7\%$ \\\hline\hline
%seq11			0,643			0,588			0,565
%seq15			0,000			0,000			0,000
\multirow{2}{*}{Average \legendMOTPDelta} & $0.957$ & $0.778$ & $\mbf{0.668}$ & $0.836$ & $0.666$ & $\mbf{0.605}$ & $0.760$ & $0.585$ & $\mbf{0.530}$ \\
 &  & $18.7\%$ & $\mbf{30.2\%}$ &  & $20.4\%$ & $\mbf{27.6\%}$ &  & $22.9\%$ & $\mbf{30.2\%}$ 
	\end{tabular}
	\caption{Results for the SRP-PHAT strategy
    (columns SRP); the one in \cite{velasco2012-F} (columns
    GMBF); and the CNN fine tuned with the sequences
    described in Table~\ref{tab:fine-tuning-material} (columns CNNf15+static).%  for sequences \seq01
    % \seq02 and \seq03 for different window sizes. Relative
    % improvements as compared to SRP-PHAT are shown below the MOTP
    % values.
}
	\label{tab:baselineResults+ft15+1+2+3}
\end{table}

%% \begin{equation}
%% \left[
%%   \begin{array}{c}
%%   MOTP \\
%%   \Delta_{r}^{MOTP} \\
%%   \end{array}
%% \right]
%% \end{equation}


%\left[  \begin{array}{c}   MOTP \\   \Delta_{r}^{MOTP} \end{array} \right]


==> table-baseline+ft15+1+2+3.tex <==
\begin{table}[H]
  \footnotesize
	\centering
	\begin{tabular}{c|cc|cc|cc}
    % \hline
    &   \multicolumn{2}{c|}{\textbf{80$ms$}}	& \multicolumn{2}{c|}{\textbf{160$ms$}} & \multicolumn{2}{c}{\textbf{320$ms$}}\\
    & GMBF & CNNf15+static & GMBF & CNNf15+static & GMBF & CNNf15+static \\\hline\hline
    \multirow{2}{*}{\seq01 \legendMOTPDelta} & $0.795$ & $\mbf{0.619}$ & $0.686$ & $\mbf{0.570}$ & $0.588$ & $\mbf{0.493}$\\
    & $22.1\%$ & $\mbf{39.3\%}$ & $24.6\%$ & $\mbf{37.4\%}$ & $29.1\%$ & $\mbf{40.6\%}$ \\\hline
    \multirow{2}{*}{\seq02 \legendMOTPDelta} & $0.864$ & $\mbf{0.685}$ & $0.759$ & $\mbf{0.603}$ & $0.694$ & $\mbf{0.554}$ \\
    & $10.0\%$ & $\mbf{28.6\%}$ & $9.6\%$ & $\mbf{28.2\%}$ & $9.9\%$ & $\mbf{28.1\%}$ \\\hline
    \multirow{2}{*}{\seq03 \legendMOTPDelta} & $\mbf{0.686}$ & $0.694$ & $\mbf{0.563}$ & $0.638$ & $\mbf{0.484}$ & $0.540$ \\
    & $\mbf{23.8\%}$ & $22.9\%$ & $\mbf{26.9\%}$ & $17.1\%$ & $\mbf{29.9\%}$ & $21.7\%$ \\\hline\hline
    % seq11			0,643			0,588			0,565
    % seq15			0,000			0,000			0,000
    \multirow{2}{*}{Average \legendMOTPDelta} & $0.778$ & $\mbf{0.668}$ & $0.666$ & $\mbf{0.605}$ & $0.585$ & $\mbf{0.530}$ \\
    & $18.7\%$ & $\mbf{30.2\%}$ & $20.4\%$ & $\mbf{27.6\%}$ & $22.9\%$ & $\mbf{30.2\%}$ 
	\end{tabular}
	\caption{Relative improvements over SRP-PHAT for strategy in \cite{velasco2012-F} (columns
    GMBF); and the CNN fine tuned with the sequences
    described in Table~\ref{tab:fine-tuning-material} (columns CNNf15+static).%  for sequences \seq01
    % \seq02 and \seq03 for different window sizes. Relative
    % improvements as compared to SRP-PHAT are shown below the MOTP
    % values.
  }
	\label{tab:baselineResults+ft15+1+2+3}
\end{table}



==> table-baseline+ft15+11+1+2+3-withsrp.tex <==
\begin{table}[H]
\footnotesize
	\centering
	\begin{tabular}{c|ccc|ccc|ccc}
%		\hline
    &   \multicolumn{3}{c|}{\textbf{80$ms$}}	& \multicolumn{3}{c|}{\textbf{160$ms$}} & \multicolumn{3}{c}{\textbf{320$ms$}}\\
    &   SRP & GMBF & CNNf15+11+static & SRP & GMBF & CNNf15+11+static & SRP & GMBF & CNNf15+11+statu \\\hline\hline
\multirow{2}{*}{\seq01 \legendMOTPDelta} & $1.020$ & $0.795$ & $\mbf{0.607}$ & $0.910$ & $0.686$ & $\mbf{0.540}$ & $0.830$ & $0.588$ & $\mbf{0.485}$\\
 &  & $22.1\%$ & $\mbf{40.5\%}$ &  & $24.6\%$ & $\mbf{40.7\%}$ &  & $29.1\%$ & $\mbf{41.6\%}$ \\\hline
\multirow{2}{*}{\seq02 \legendMOTPDelta} & $0.960$ & $0.864$ & $\mbf{0.669}$ & $0.840$ & $0.759$ & $\mbf{0.579}$ & $0.770$ & $0.694$ & $\mbf{0.545}$ \\
 &  & $10.0\%$ & $\mbf{30.3\%}$ &  & $9.6\%$ & $\mbf{31.1\%}$ &  & $9.9\%$ & $\mbf{29.2\%}$ \\\hline
\multirow{2}{*}{\seq03 \legendMOTPDelta} & $0.900$ & $\mbf{0.686}$ & $0.707$ & $0.770$ & $\mbf{0.563}$ & $0.617$ & $0.690$ & $\mbf{0.484}$ & $0.501$ \\
 &  & $\mbf{23.8\%}$ & $21.4\%$ &  & $\mbf{26.9\%}$ & $19.9\%$ &  & $\mbf{29.9\%}$ & $27.4\%$ \\\hline\hline
%seq11			0,643			0,588			0,565
%seq15			0,000			0,000			0,000
\multirow{2}{*}{Average \legendMOTPDelta} & $0.957$ & $0.778$ & $\mbf{0.664}$ & $0.836$ & $0.666$ & $\mbf{0.581}$ & $0.760$ & $0.585$ & $\mbf{0.511}$ \\
 &  & $18.7\%$ & $\mbf{30.6\%}$ &  & $20.4\%$ & $\mbf{30.6\%}$ &  & $22.9\%$ & $\mbf{32.8\%}$ 
	\end{tabular}
	\caption{Results for the standard SRP-PHAT strategy
    (columns SRP); the one in \cite{velasco2012-F} (columns
    GMBF); and the CNN fine tuned with the sequences
    described in Table~\ref{tab:fine-tuning-material} (columns CNNf15+11+static) % for sequences \seq01
    % \seq02 and \seq03 for different window sizes. Relative
    % improvements as compared to SRP-PHAT are shown below the MOTP
    % values.
}
	\label{tab:baselineResults+ft15+1+2+3}
\end{table}

%% \begin{equation}
%% \left[
%%   \begin{array}{c}
%%   MOTP \\
%%   \Delta_{r}^{MOTP} \\
%%   \end{array}
%% \right]
%% \end{equation}


%\left[  \begin{array}{c}   MOTP \\   \Delta_{r}^{MOTP} \end{array} \right]


==> table-baseline+ft15+11-withsrp.tex <==
\begin{table}[H]
\footnotesize
	\centering
	\begin{tabular}{c|ccc|ccc|ccc}
%		\hline
    &   \multicolumn{3}{c|}{\textbf{80$ms$}}	& \multicolumn{3}{c|}{\textbf{160$ms$}} & \multicolumn{3}{c}{\textbf{320$ms$}}\\
    &   SRP & GMBF & CNNf15+11 & SRP & GMBF & CNNf15+11 & SRP & GMBF & CNNf15+11 \\\hline\hline
\multirow{2}{*}{\seq01 \legendMOTPDelta} & $1.020$ & $\mbf{0.795}$ & $0.805$ & $0.910$ & $\mbf{0.686}$ & $0.750$ & $0.830$ & $\mbf{0.588}$ & $0.706$\\
 &  & $\mbf{22.1\%}$ & $21.1\%$ &  & $\mbf{24.6\%}$ & $17.6\%$ &  & $\mbf{29.1\%}$ & $14.9\%$\\\hline
\multirow{2}{*}{\seq02 \legendMOTPDelta} & $0.960$ & $0.864$ & $\mbf{0.809}$ & $0.840$ & $0.759$ & $\mbf{0.716}$ & $0.770$ & $\mbf{0.694}$ & $0.712$\\
 &  & $10.0\%$ & $\mbf{15.7\%}$ &  & $9.6\%$ & $\mbf{14.8\%}$ &  & $9.9\%$ & $7.5\%$\\\hline
\multirow{2}{*}{\seq03 \legendMOTPDelta} & $0.900$ & $\mbf{0.686}$ & $0.792$ & $0.770$ & $\mbf{0.563}$ & $0.732$ & $0.690$ & $\mbf{0.484}$ & $0.692$\\
 &  & $\mbf{23.8\%}$ & $12.0\%$ &  & $\mbf{26.9\%}$ & $4.9\%$ &  & $\mbf{29.9\%}$ & $-0.3\%$\\\hline\hline
%seq11			0,000			0,000			0,000
%seq15			0,000			0,000			0,000
\multirow{2}{*}{Average \legendMOTPDelta} & $0.957$ & $\mbf{0.778}$ & $0.802$ & $0.836$ & $\mbf{0.666}$ & $0.732$ & $0.760$ & $\mbf{0.585}$ & $0.703$\\
 &  & $\mbf{18.7\%}$ & $16.2\%$ &  & $\mbf{20.4\%}$ & $12.4\%$ &  & $\mbf{22.9\%}$ & $7.5\%$\\
	\end{tabular}
	\caption{Results for the SRP-PHAT strategy
    (columns SRP); the one in \cite{velasco2012-F} (columns
    GMBF); and the CNN fine tuned with sequences
    \seq15 and \seq11 (columns CNNf15+11) % for sequences \seq01,
    % \seq02 and \seq03 for different window sizes. Relative
    % improvements as compared to SRP-PHAT are shown below the MOTP
    % values.
}
	\label{tab:baselineResults+ft15+11}
\end{table}

%% \begin{equation}
%% \left[
%%   \begin{array}{c}
%%   MOTP \\
%%   \Delta_{r}^{MOTP} \\
%%   \end{array}
%% \right]
%% \end{equation}


%\left[  \begin{array}{c}   MOTP \\   \Delta_{r}^{MOTP} \end{array} \right]


==> table-baseline+ft15-withsrp.tex <==
\begin{table}[H]
\footnotesize
	\centering
	\begin{tabular}{c|ccc|ccc|ccc}
%		\hline
    &   \multicolumn{3}{c|}{\textbf{80$ms$}}	& \multicolumn{3}{c|}{\textbf{160$ms$}} & \multicolumn{3}{c}{\textbf{320$ms$}}\\
    &   SRP & GMBF & CNNf15 & SRP & GMBF & CNNf15 & SRP & GMBF & CNNf15 \\\hline\hline
    \multirow{2}{*}{\seq01 \legendMOTPDelta} & $1.020$ & $\mbf{0.795}$ & $0.875$ & $0.910$ & $\mbf{0.686}$ & $0.833$ & $0.830$ & $\mbf{0.588}$ & $0.777$ \\
    &  & $\mbf{22.1\%}$ & $14.2\%$ &  & $\mbf{24.6\%}$ & $8.5\%$ &  & $\mbf{29.1\%}$ & $6.4\%$ \\\hline
    \multirow{2}{*}{\seq02 \legendMOTPDelta} & $$0.960$$ & $0.864$ & $\mbf{0.839}$ & $0.840$ & $\mbf{0.759}$ & $0.801$ & $0.770$ & $\mbf{0.694}$ & $0.731$ \\
    &  & $10.0\%$ & $\mbf{12.6\%}$ &  & $\mbf{9.6\%}$ & $4.6\%$ &  & $\mbf{9.9\%}$ & $5.1\%$ \\\hline
    \multirow{2}{*}{\seq03 \legendMOTPDelta} & $0.900$ & $\mbf{0.686}$ & $0.835$ & $0.770$ & $\mbf{0.563}$ & $0.806$ & $0.690$ & $\mbf{0.484}$ & $0.734$ \\
    &  & $\mbf{}$23.8\%$$ & $7.2\%$ &  & $\mbf{26.9\%}$ & -$4.7\%$ &  & $\mbf{29.9\%}$ & -$6.4\%$ \\\hline\hline
    % seq11			0,884			0,923			0,843
    % seq15			0,000			0,000			0,000
    \multirow{2}{*}{Average \legendMOTPDelta} & $0.957$ & $\mbf{0.778}$ & $0.849$ & $0.836$ & $\mbf{0.666}$ & $0.813$ & $0.760$ & $\mbf{0.585}$ & $0.746$ \\
    &  & $\mbf{18.7\%}$ & $11.3\%$ &  & $\mbf{20.4\%}$ & $2.8\%$ &  & $\mbf{22.9\%}$ & $1.8\%$ \\%\hline
	\end{tabular}
	\caption{Results for the SRP-PHAT strategy
    (columns SRP); the one in \cite{velasco2012-F} (columns
    GMBF); and the CNN fine tuned with sequence \seq15
    (columns CNNf15).%  for sequences \seq01,
    % \seq02 and \seq03 for different window sizes. Relative
    % improvements as compared to SRP-PHAT are shown below the MOTP
    % values.
}
	\label{tab:baselineResults+ft15}
\end{table}

%% \begin{equation}
%% \left[
%%   \begin{array}{c}
%%   MOTP \\
%%   \Delta_{r}^{MOTP} \\
%%   \end{array}
%% \right]
%% \end{equation}


%\left[  \begin{array}{c}   MOTP \\   \Delta_{r}^{MOTP} \end{array} \right]


==> table-baseline+ft15vstr15-withsrp.tex <==
\begin{table}[H]
\footnotesize
	\centering
	\begin{tabular}{c|ccc|ccc|ccc}
%		\hline
    &   \multicolumn{3}{c|}{\textbf{80$ms$}}	& \multicolumn{3}{c|}{\textbf{160$ms$}} & \multicolumn{3}{c}{\textbf{320$ms$}}\\
    &   SRP & CNNt15 & CNNf15 & SRP & CNNt15 & CNNf15 & SRP & CNNt15 & CNNf15 \\\hline\hline
    \multirow{2}{*}{\seq01 \legendMOTPDelta} & $1.020$ & $1.009$ & $\mbf{0.875}$ & $0.910$ & $0.949$ & $\mbf{0.833}$ & $0.833$ & $1.0009$ & $\mbf{0.777}$ \\
    &  & $1.1\%$ & $\mbf{14.2\%}$ &  & $-4.3\%$ & $\mbf{8.5\%}$ &  & $-21.6\%$ & $\mbf{6.4\%}$ \\\hline
    \multirow{2}{*}{\seq02 \legendMOTPDelta} & $0.960$ & $\mbf{0.807}$ & $0.839$ & $0.840$ & $\mbf{0.767}$ & $0.801$ & $0.770$ & $0.807$ & $\mbf{0.731}$ \\
    &  & $\mbf{15.9\%}$ & $12.6\%$ &  & $\mbf{8.7\%}$ & $4.6\%$ &  & $-4.8\%$ & $\mbf{5.1\%}$ \\\hline
    \multirow{2}{*}{\seq03 \legendMOTPDelta} & $0.900$ & $0.935$ & $\mbf{0.835}$ & $0.770$ & $0.911$ & $\mbf{0.806}$ & $0.690$ & $0.936$ & $\mbf{0.734}$ \\
    &  & $-3.9\%$ & $\mbf{7.2\%}$ &  & $-18.3\%$ & $\mbf{-4.7\%}$ &  & $-35.7\%$ & $\mbf{-6.4\%}$ \\\hline\hline
    % seq11			0,884			0,923			0,843
    % seq15			0,000			0,000			0,000
    \multirow{2}{*}{Average \legendMOTPDelta} & $0.957$ & $0.915$ & $\mbf{0.849}$ & $0.836$ & $0.875$ & $\mbf{0.813}$ & $0.760$ & $0.916$ & $\mbf{0.746}$ \\
    &  & $4.3\%$ & $\mbf{11.3\%}$ &  & $-4.6\%$ & $\mbf{2.8\%}$ &  & $-20.6\%$ & $\mbf{1.8\%}$ \\%\hline
	\end{tabular}
	\caption{Results for the SRP-PHAT strategy
    (columns SRP) and the CNN, either trained from scratch
    with sequence \seq15 (columns CNNt15) or fine tuned with sequence \seq15
    (columns CNNf15).%  for sequences \seq01,
    % \seq02 and \seq03 for different window sizes. Relative
    % improvements as compared to SRP-PHAT are shown below the MOTP
    % values.
}
	\label{tab:baselineResults+ft15vstr15}
\end{table}

%% \begin{equation}
%% \left[
%%   \begin{array}{c}
%%   MOTP \\
%%   \Delta_{r}^{MOTP} \\
%%   \end{array}
%% \right]
%% \end{equation}


%\left[  \begin{array}{c}   MOTP \\   \Delta_{r}^{MOTP} \end{array} \right]


==> table-baseline-withsrp.tex <==
\begin{table}[H]
\footnotesize
	\centering
	\begin{tabular}{c|ccc|ccc|ccc}
%		\hline
		      &   \multicolumn{3}{c|}{\textbf{80$ms$}}	& \multicolumn{3}{c|}{\textbf{160$ms$}} & \multicolumn{3}{c}{\textbf{320$ms$}}\\
   		    &   SRP & GMBF & CNN & SRP & GMBF & CNN & SRP & GMBF & CNN \\\hline\hline
    \multirow{2}{*}{\seq01 \legendMOTPDelta} &             $1.020$ &    $\mbf{0.795}$ &  $1.615$     & $0.910$ &    $0.686$ &     $1.526$ & $0.830$ &    $\mbf{0.588}$ &     $1.464$ \\
          &    & $\mbf{22.1\%}$ &  $-58.3\%$ &       & $\mbf{24.6\%}$ & $-67.7\%$ &       & $\mbf{29.1\%}$ & $-76.4\%$ \\\hline
    \multirow{2}{*}{\seq02 \legendMOTPDelta} &             $0.960$ & $\mbf{0.864}$    &      $2.124$ & $0.840$ & $\mbf{0.759}$    &     $1.508$ & $0.770$ & $\mbf{0.694}$    & $1.318$     \\
          &    & $\mbf{10.0\%}$ & $-121.3\%$ &       & $\mbf{9.6\%}$  & $-79.5\%$ &       & $\mbf{9.9\%}$  & $-71.2\%$ \\\hline
    \multirow{2}{*}{\seq03 \legendMOTPDelta} &  $0.900$ & $\mbf{0.686}$ & $1.559$ & $0.770$ & $\mbf{0.563}$ & $1.419$ & $0.690$ & $\mbf{0.484}$ & $1.379$\\
          &    & $\mbf{23.8\%}$ & $-73.2\%$ &  & $\mbf{26.9\%}$ & $-84.3\%$ &  & $\mbf{29.9\%}$ & $-99.9\%$\\\hline\hline
%    \multirow{2}{*}{seq11 \legendMOTPDelta} &   &  & $1.360$ &  &  & $1.154$ &  &  & $1.279$\\
%          &    &  &  &  &  &  &  &  & \\\hline
%    \multirow{2}{*}{seq15 \legendMOTPDelta} &   &  & $1.879$ &  &  & $1.862$ &  &  & $1.763$\\
%          &    &  &  &  &  &  &  &  &\\\hline
\multirow{2}{*}{Average \legendMOTPDelta}  & $0.957$ & $\mbf{0.778}$ & $1.763$ & $0.836$ & $\mbf{0.666}$ & $1.481$ & $0.760$ & $\mbf{0.585}$ & $1.385$\\
 &  & $\mbf{18.7\%}$ & $-84.3\%$ &  & $\mbf{20.4\%}$ & $-77.1\%$ &  & $\mbf{22.9\%}$ & $-82.3\%$\\%\hline
	\end{tabular}
	\caption{Baseline results for the SRP-PHAT strategy
    (columns SRP); the one in \cite{velasco2012-F} (columns
    GMBF), and the CNN trained with synthetic data without applying the
    fine-tuning procedure (columns CNN) for sequences \seq01,
    \seq02 and \seq03 for different window sizes. Relative
    improvements as compared to SRP-PHAT are shown below the MOTP
    values.}
	\label{tab:baselineResults}
\end{table}

%% \begin{equation}
%% \left[
%%   \begin{array}{c}
%%   MOTP \\
%%   \Delta_{r}^{MOTP} \\
%%   \end{array}
%% \right]
%% \end{equation}


%\left[  \begin{array}{c}   MOTP \\   \Delta_{r}^{MOTP} \end{array} \right]


==> table-ft15+1.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		& \multicolumn{2}{c|}{\textbf{80$ms$}}	& \multicolumn{2}{c|}{\textbf{160$ms$}} & \multicolumn{2}{c|}{\textbf{320$ms$}}\\
		& GMBF-SC & EE-CNN & GMBF-SC & EE-CNN & GMBF-SC & EE-CNN \\\hline
		seq02 &  $10.0\%$ &  $\mbf{28.13\%}$ &  $9.6\%$ &  $\mbf{17.86\%}$ &  $\mbf{9.9\%}$ &  $7.79\%$\\\hline
		seq03 &  $\mbf{23.8\%}$ &  $23.3\%$ &  $\mbf{26.9\%}$ &  $12.99\%$ &  $\mbf{9.9\%}$ &  $5.79\%$\\\hline
	\end{tabular}
	\caption{Relative improvement of $MOTP$ results ($\Delta_{r}^{MOTP}$)
    for sequences \texttt{seq2} and \texttt{seq3} for different window
    sizes and fine tuning with sequences \texttt{seq1} and \texttt{seq15}.}
	\label{tab:FTseq15}
\end{table}


==> table-ft15+2.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		& \multicolumn{2}{c|}{\textbf{80$ms$}}	& \multicolumn{2}{c|}{\textbf{160$ms$}} & \multicolumn{2}{c|}{\textbf{320$ms$}}\\
		& GMBF-SC & EE-CNN & GMBF-SC & EE-CNN & GMBF-SC & EE-CNN \\\hline
		seq01 &  $22.1\%$ &  $\mbf{28.43\%}$ &  $\mbf{24.6\%}$ &  $21.98\%$ &  $29.1\%$ &  $\mbf{29.92\%}$\\\hline
		seq03 &  $\mbf{23.8\%}$ &  $14.44\%$ &  $\mbf{26.9\%}$ &  $7.79\%$ &  $9.9\%$ &  $\mbf{11.59\%}$\\\hline
	\end{tabular}
	\caption{Relative improvement of $MOTP$ results ($\Delta_{r}^{MOTP}$)
    for sequences \texttt{seq1} and \texttt{seq2} for different window
    sizes and fine tuning with sequences \texttt{seq2} and \texttt{seq15}.}
	\label{tab:FTseq15seq2}
\end{table}



==> table-ft15+2improvements-simple.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c|c|c|c}
		\toprule
		& \textbf{80$ms$}	& \textbf{160$ms$} & \textbf{320$ms$}\\
		\midrule
		seq01 & $\Delta_{r}^{MOTP}$ = 28,43\% &  $\Delta_{r}^{MOTP}$ = 21.98\% &  $\Delta_{r}^{MOTP}$ = 29.92\%\\
		\midrule
		seq03 & $\Delta_{r}^{MOTP}$ = 14.44\% &  $\Delta_{r}^{MOTP}$ = 7.79\% &  $\Delta_{r}^{MOTP}$ = 11.59\%\\
	\end{tabular}
	\caption{Relative improvement of $MOTP$ results for sequences \texttt{seq1} and \texttt{seq3} for different window sizes and fine tuning with sequence \texttt{seq15} and sequence \texttt{seq2}.}
	\label{tab:FTseq15seq2}
\end{table}


==> table-ft15+3.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		& \multicolumn{2}{c|}{\textbf{80$ms$}}	& \multicolumn{2}{c|}{\textbf{160$ms$}} & \multicolumn{2}{c|}{\textbf{320$ms$}}\\
		& GMBF-SC & EE-CNN & GMBF-SC & EE-CNN & GMBF-SC & EE-CNN \\\hline
		seq01 &  $22.1\%$ &  $\mbf{36.27\%}$ &  $24.6\%$ &  $\mbf{35.16\%}$ &  $29.1\%$ &  $\mbf{39.76\%}$\\\hline
		seq02 &  $10.0\%$ &  $\mbf{23.3\%}$ &   $ 9.6\%$ &  $\mbf{18.18\%}$ &  $9.9\%$ &  $\mbf{15.94\%}$\\\hline
	\end{tabular}
	\caption{Relative improvement of $MOTP$ results ($\Delta_{r}^{MOTP}$)
    for sequences \texttt{seq1} and \texttt{seq2} for different window
    sizes and fine tuning with sequences \texttt{seq3} and \texttt{seq15}.}
	\label{tab:FTseq15seq3}
\end{table}



==> table-ft15+3improvements-simple.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c|c|c|c}
		\toprule
		& \textbf{80$ms$}	& \textbf{160$ms$} & \textbf{320$ms$}\\
		\midrule
		seq01 & $\Delta_{r}^{MOTP}$ = 36.27\% &  $\Delta_{r}^{MOTP}$ = 35.16\% &  $\Delta_{r}^{MOTP}$ = 39.76\%\\
		\midrule
		seq02 & $\Delta_{r}^{MOTP}$ = 23.3\% &  $\Delta_{r}^{MOTP}$ = 18.18\% &  $\Delta_{r}^{MOTP}$ = 15.94\%\\
	\end{tabular}
	\caption{Relative improvement of $MOTP$ results for sequences \texttt{seq1} and \texttt{seq2} for different window sizes and fine tuning with sequence \texttt{seq15} and sequence \texttt{seq3}.}
	\label{tab:FTseq15seq3}
\end{table}


==> table-ft15.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		& \multicolumn{2}{c|}{\textbf{80$ms$}}	& \multicolumn{2}{c|}{\textbf{160$ms$}} & \multicolumn{2}{c|}{\textbf{320$ms$}}\\
		& GMBF-SC & EE-CNN & GMBF-SC & EE-CNN & GMBF-SC & EE-CNN \\\hline
		seq01 &  $\mbf{22.1\%}$ &  $13.73\%$ &  $\mbf{24.6\%}$ &  $8.79\%$ &  $\mbf{29.1\%}$ &  $7.22\%$\\\hline
		seq02 &  $10.0\%$ &  $\mbf{12.50\%}$ &  $\mbf{9.6\%}$ &  $4.76\%$ &  $\mbf{9.9\%}$ &  $5.19\%$\\\hline
		seq03 &  $\mbf{23.8\%}$ &  $6.66\%$ &  $\mbf{26.9\%}$ &  $0.00\%$ &  $\mbf{29.9\%}$ &  $0.00\%$\\\hline
	\end{tabular}
	\caption{Relative improvement of $MOTP$ results ($\Delta_{r}^{MOTP}$) for sequences \texttt{seq1}, \texttt{seq2} and \texttt{seq3} for different window sizes and fine tuning with sequence \texttt{seq15}.}
	\label{tab:FTseq15}
\end{table}


==> table-ft15improvements-simple.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c|c|c|c}
		\toprule
		& \textbf{80$ms$}	& \textbf{160$ms$} & \textbf{320$ms$}\\
		\midrule
		seq01 & $\Delta_{r}^{MOTP}$ = 13.73\% &  $\Delta_{r}^{MOTP}$ = 8.79\% &  $\Delta_{r}^{MOTP}$ = 7.22\%\\
		\midrule
		seq02 & $\Delta_{r}^{MOTP}$ = 12.50\% &  $\Delta_{r}^{MOTP}$ = 4.76\% &  $\Delta_{r}^{MOTP}$ = 5.19\%\\
		\midrule
		seq03 & $\Delta_{r}^{MOTP}$ = 6.66\% &  $\Delta_{r}^{MOTP}$ = 0.00\% &  $\Delta_{r}^{MOTP}$ = 0.00\%\\
	\end{tabular}
	\caption{Relative improvement of $MOTP$ results for sequences \texttt{seq1}, \texttt{seq2} and \texttt{seq3} for different window sizes and fine tuning with sequence \texttt{seq15}.}
	\label{tab:FTseq15}
\end{table}


==> table-improvements-simple.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c|c|c|c}
		\toprule
		& \textbf{80$ms$}	& \textbf{160$ms$} & \textbf{320$ms$}\\
		\midrule
		seq01 & $\Delta_{r}^{MOTP}$ = 22.1\% & $\Delta_{r}^{MOTP}$ = 24.6\% & $\Delta_{r}^{MOTP}$ = 29.1\%\\
		\midrule
		seq02 & $\Delta_{r}^{MOTP}$ = 10.0\% & $\Delta_{r}^{MOTP}$ = 9.6\% & $\Delta_{r}^{MOTP}$ = 9.9\%\\
		\midrule
		seq03 & $\Delta_{r}^{MOTP}$ = 23.8\% & $\Delta_{r}^{MOTP}$ = 26.9\% & $\Delta_{r}^{MOTP}$ = 29.9\%\\
	\end{tabular}
	\caption{Relative improvement of $MOTP$ results for sequences \texttt{seq1}, \texttt{seq2} and \texttt{seq3} for different window sizes from \cite{JoseVelascoThesis2017}.}% cite was \cite{JoseThesis}
	\label{tab:JoseResults}
\end{table}

